Novice Type Error Diagnosis with Natural Language Models

Strong static type systems help programmers eliminate many errors without much burden of supplying type annotations. However, this flexibility makes it highly non-trivial to diagnose ill-typed programs, especially for novice programmers. Compared to classic constraint solving and optimization-based approaches, the data-driven approach has shown great promise in identifying the root causes of type errors with higher accuracy. Instead of relying on hand-engineered features, this work explores natural language models for type error localization, which can be trained in an end-to-end fashion without requiring any features. We demonstrate that, for novice type error diagnosis, the language model-based approach significantly outperforms the previous state-of-the-art data-driven approach. Specifically, our model could predict type errors correctly 62% of the time, outperforming the state-of-the-art Nate's data-driven model by 11%, in a more rigorous accuracy metric. Furthermore, we also apply structural probes to explain the performance difference between different language models.

==> bib.tex <==
\bibliography{citation}
\begin{thebibliography}{8}
\bibitem{sherrloc}
Loncaric, C., Chandra, S., Schlesinger, C., Sridharan, M.: A practical framework for type inference error explanation. In: Proceedings of the 2016 ACM SIGPLAN International Conference on Object-Oriented Programming, Systems, Languages, and Applications, pp. 781--799. Association for Computing Machinery, New York, New York (2016). \doi{10.1145/2983990.2983994}

\bibitem{nate}
Seidel, E.L., Sibghat, H., Chaudhuri, K., Weimer, W., Jhala, R.: Learning to blame: localizing novice type errors with data-driven diagnosis. Proceedings of the ACM on Programming Languages \textbf{1}(OOPSLA), 60:1--60:27 (2017).
\doi{10.1145/3138818}


\bibitem{attention}
Vaswani, A., Shazeer, N., Parmar, N., Uszkoreit, J., Jones, L., Gomez, A.N., Kaiser, Ł., Polosukhin, I.: Attention is all you need. In: Proceedings of the 31st International Conference on Neural Information Processing Systems (NIPS'17), pp. 6000--6010. Curran Associates Inc., Red Hook, New York (2017).
\doi{10.5555/3295222.3295349}



\bibitem{bert}
Devlin, J., Chang, M., Lee, K., Toutanova, K.: BERT: Pre-training of deep bidirectional transformers for language understanding. In: Proceedings of the 2019 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies, pp. 4171--4186. Association for Computational Linguistics, Minneapolis, Minnesota (2019).
\doi{10.18653/v1/N19-1423}

\bibitem{gpt-2}
Radford, A., Wu, J., Child, R., Luan, D., Amodei, D., Sutskever, I.: Language models are unsupervised multitask learners. OpenAI blog \textbf{1}(8), 9 (2019)

\bibitem{gpt-3}
Brown, T., Mann, B., Ryder, N., Subbiah, M., et al.: Language models are few-shot learners. Advances in neural information processing systems \textbf{33}, 1877--1901 (2020)


\bibitem{joosten}
Joosten, S., Berg, K.V.D., Hoeven, G.V.D.: Teaching functional programming to first-year students. Journal of Functional Programming \textbf{3}(01), 49--65 (1993)

\bibitem{mycroft}
Zhang, D., Myers, A.C.: Toward general diagnosis of static errors. In: Proceedings of the 41st ACM SIGPLAN-SIGACT Symposium on Principles of Programming Languages (POPL'14), pp. 569--581. Association for Computing Machinery, New York, New York (2014). \doi{10.1145/2578855.2535870.}

\bibitem{PLDI}
Jose, M., Majumdar, R.: Cause clue clauses: error localization using maximum satisfiability. In: Proceedings of the 32nd ACM SIGPLAN Conference on Programming Language Design and Implementation (PLDI '11), pp. 437--446. Association for Computing Machinery, New York, New York (2011).
\doi{10.1145/1993498.1993550}

\bibitem{probe}
Christopher D.M., Kevin C., John H., Urvashi K., Omer L.: Emergent linguistic structure in artificial neural networks trained by self-supervision. Proceedings of the National Academy of Sciences \textbf{117}(48), 30046--30054 (2020).
\doi{10.1073/pnas.1907367117}

\bibitem{schuster97bidirectional}
Schuster, M., Paliwal, K.K.: Bidirectional recurrent neural networks. IEEE Transactions on Signal Processing \textbf{45}(11), 2673--2681 (1997)

\bibitem{Keefe}
O’Keefe, C., Lansky, D., Clark, J., Payne, C.: Comment regarding request for comments on intellectual property protection for artificial intelligence innovation (2019).
\url{https://perma.cc/ZS7G-2QWF}

\bibitem{guided}
Chen, S., Erwig, M.: Guided type debugging. In: Codish, M., Sumii, E. (eds) Functional and Logic Programming. FLOPS (2014). Lecture Notes in Computer Science, vol 8475. Springer, Cham (2014). \doi{10.1007/978-3-319-07151-0_3}

\bibitem{minimum}
Pavlinovic, Z., King, T., Wies, T.: Finding minimum type error sources. SIGPLAN \textbf{49}(10), 525--542 (2014). \doi{10.1145/2660193.2660230}

\bibitem{maximum}
Jose, M., Majumdar, R.: Cause clue clauses: Error localization using maximum satisfiability. SIGPLAN \textbf{46}(6), 437--446 (2011). \doi{10.1145/1993316.1993550} 

\bibitem{dynamic}
Seidel, E.L., Jhala, R., Weimer, W.: Dynamic witnesses for static type errors (or, Ill-Typed programs usually go wrong). In: Proceedings of the 21st ACM SIGPLAN International Conference on Functional Programming (ICFP 2016), pp. 228--242. Association for Computing Machinery, New York, New York (2016). \doi{10.1145/2951913.2951915}.

\bibitem{transfer}
Zhuang, F., Qi, Z., Duan, K., Xi, D., et al.: A comprehensive survey on transfer learning. Proceedings of the IEEE \textbf{109}(1), 43--76 (2021). \doi{10.48550/ARXIV.1911.02685}

\bibitem{generalization}
Neyshabur, B., Bhojanapalli, S., McAllester, D., Srebro, N.: Exploring generalization in deep learning. In: Proceedings of the 31st International Conference on Neural Information Processing Systems (NIPS'17), pp. 5949--5958. Curran Associates Inc., Red Hook, New York (2017). \doi{10.5555/3295222.3295344}



\bibitem{Bilstm}
Schuster, M., &amp; Paliwal, K. K. (1997). Bidirectional recurrent neural networks. IEEE Transactions on Signal Processing, 45(11), 2673–2681. \url{https://doi.org/10.1109/78.650093}


\iffalse
Examples
\bibitem{ref_article1}
Author, F.: Article title. Journal \textbf{2}(5), 99--110 (2016)

\bibitem{ref_lncs1}
Author, F., Author, S.: Title of a proceedings paper. In: Editor,
F., Editor, S. (eds.) CONFERENCE 2016, LNCS, vol. 9999, pp. 1--13.
Springer, Heidelberg (2016). \doi{10.10007/1234567890}

\bibitem{ref_book1}
Author, F., Author, S., Author, T.: Book title. 2nd edn. Publisher,
localization (1999)

\bibitem{ref_proc1}
Author, A.-B.: Contribution title. In: 9th International Proceedings
on Proceedings, pp. 1--2. Publisher, localization (2010)

\bibitem{ref_url1}
LNCS Homepage, \url{http://www.springer.com/lncs}. Last accessed 4
Oct 2017
\end{thebibliography}


==> code-examples/code-1.tex <==

\begin{minipage}{7.2cm}
%\begin{lstlisting} [numbers=none]
\begin{lstlisting} [numbers=none,escapechar=\%]
let sumList xs = 
  match xs with 
  | [] -> []
  | h :: t -> h + sumList t
  
  | % \underline{\ \ \ \ \ \ \ \circled{1}  \ \ \ \ \ \ \ }  % 
  | % \underline{\ \ \ \ \ \ \ \circled{2}  \ \ \ \ \ \ \ }  %
\end{lstlisting}
\end{minipage}


==> code-examples/comparison.tex <==
\definecolor{lightblue}{rgb}{.0,.95,1.05}
\definecolor{lightgreen}{rgb}{0.79,2.50,0.79}
\definecolor{lightpurple}{rgb}{0.64,0.93,0.30}

% \lstset
% { %Formatting for code in appendix
%     numbers=none,
% }

\begin{minipage}{14.2cm}
% \begin{lstlisting} [numbers=none]
\begin{lstlisting} [escapechar=\%, numbers=none]
let rec clone x n = if n <= 0 then [] else x :: (clone x (n - 1));;

let rec helper x = 
  if x = 0 then 1 else 10 * (helper (x - 1));;

let padZero l1 l2 =
  if (List.length l1) < (List.length l2)
  then ((%\sethlcolor{yellow} \textcolor{red}{\hl{clone}} % "0" %\sethlcolor{yellow} \textcolor{red}{\hl{List.length}}% l2) - (List.length l1)) :: l1
  else ((%\sethlcolor{yellow} \textcolor{red}{\hl{clone}}% "0" List.length l1) - (List.length l2)) :: l2;;
\end{lstlisting}
\end{minipage}

\begin{minipage}{14.2cm}
%\begin{lstlisting} [numbers=none]
\begin{lstlisting} [escapechar=\%, numbers=none]
let rec clone x n = if n <= 0 then [] else x :: (clone x (n - 1));;


let padZero l1 l2 =
  if (List.length l1) < (List.length l2)
  then %\sethlcolor{lightblue} \textcolor{black}{\hl{(((clone 0 ((List.length l2) - (List.length l1))) @ l1), l2)}}%
  else %\sethlcolor{lightblue} \textcolor{black}{\hl{(((clone 0 ((List.length l1) - (List.length l2))) @ l2), l1)}}%;;

\end{lstlisting}
\end{minipage}

\begin{minipage}{14.2cm}
% \begin{lstlisting} [numbers=none]
\begin{lstlisting} [escapechar=\%, numbers=none]
let rec sumList xs =
  match xs with
  | [] -> %\sethlcolor{yellow} \textcolor{red}{\hl{[]}}%         (* type error *)
  | h :: t -> h + %\blueuwave{sumList t}% ;;
  %\sethlcolor{red}\textcolor{white}{\hl{This expression has type 'a list
       but an expression was expected of type int}}%
\end{lstlisting}
\end{minipage}

\begin{minipage}{14.2cm}
% \begin{lstlisting} [numbers=none]
\begin{lstlisting} [escapechar=\%, numbers=none]
let rec sumList xs =
  match xs with
  | [] -> %\sethlcolor{lightblue} \textcolor{black}{\hl{0}}%         (* fixed *)
  | h :: t -> h + sumList t ;;
\end{lstlisting}
\end{minipage}

==> overview.tex <==
\section{Challenges}
\label{sec: overview}
\textbf{\textit{Supervision}}
As a data-driven approach, our language models learn how to localize type error in a supervised learning fashion. This means we need to provide supervision or labeled dataset to facilitate models' learning. In our problem, supervision should consist of a sufficiently large number of ill-typed programs along with the correct location of type error. To make such a dataset which covers many possible type error program instances, we have to collect ill-typed programs and annotate the error location manually. 

% This, however, is a challenging task to do. 

% We show how to address this issue by leverage \nate's dataset in Section~\ref{sec: evaluation}.

\textbf{\textit{Quantifying prediction on multiple type errors}}
\nate has previously defined a top-three accuracy metric by picking three top-level predictions as probable error locations. This helps to quantify the performance of localizing multiple errors. \nate's best top-3 accuracy has reached over 90\% with this metric; however, if there are more than 3 spans/errors in the ground truth, such metric would blocks us from seeing the true performance of models when predicting multiple errors. 

% We then adjust this metric by setting a threshold defaults to 0.5, which as long as a token or span has probability greater than 50\%, we place it in the prediction set.

% Method to find the type-error ground truth of a given program. They split a program into multiple span sets that is either \textcolor{red}{'changed spans', 'type error slices', or 'all spans'} where a span can be a sub-span of others and belong to more than one set. \textcolor{red}{NATE claims that type error only happens at location where the ill-typed programs differs from its fixed version, and the expression that is one of the causes of the type conflict.} This is exactly the overlap between the first two types of span. We reckon this to be an excellent method, except it does raise problems when programs get split into spans.


%Since we discover that these problems occur 29.1\% among 2365 cases
%\textbf{\textit{Solution: }}We resolve these through simply taking the intersection when two spans are not the same, whether we are finding the ground truth or matching predictions to it. Therefore, spans to us are consecutive token string from the program. By counting the number of hit, predicted and ground-truth tokens, we can get a more precised accuracy rather than just 0\%(missed) or 100\%(hit). Notice all models in this paper follows this accuracy metric,so data from NATE will be recalculated and look different. \\



%To make the accuracy calculation more reasonable, we divide the spans into tokens. By using these tokens to calculate intersection of two span sets and compare the predicted tokens with true type error position, the accuracy we got will be more fair and precise. More specifically, for the above program, NATE gets a 100\% accuracy, while we get an accuracy of 4.65\% in our way.


==> temp/tmp.tex <==
\begin{figure}[htbp]
\centerline{Figures/\includegraphics[width=\textwidth, height =5cm]{Figures/EX2.1.png}}
\caption{Example code 1.1}
\label{fig:biased case p2}
\end{figure}

Here is one example where NATE evaluates the accuracy of prediction to 100\%, however, we think it should be much lower. To clarify, we first introduce how NATE calculate the prediction accuracy. \textcolor{red}{It looks through the program's \textit{changed} span set and \textit{type error slice} for identical spans as its ground truth.} This is yet not precisely the overlap between the two spans since intersections are disregarded. For example in Figure \ref{fig:biased case p2}, we highlight the \textit{type error slice} yellow and \textit{changed span} \textcolor{red}{red[?]}. The two spans are merely different by a function signature, \textit{let add (l1,l2) =}, and their intersection is precisely the error source if we compare it to its fixed version on the right half of the figure. However, because intersections do not count, NATE's models will miss this part of the ground truth which would greatly impact the accuracy.
%These They assume the position of type error is the intersect of these two span set and predict the possible span where type error happens. Then they choose three spans with the top 3 possibility and compare with the intersection.\\
%The first problem takes place when they get the intersection of the two span sets. As we can see in \textcolor{cyan}{Figure}, suppose yellow part represent a span in \textit{changed} set and orange part is a span in \textit{type error slice}. It is clear that orange is overlapped code span, however, NATE does not treat is as an intersection since, as they use "==" to find the overlap, it only includes spans that are exactly same in two sets. The situation is even worse as the each span might be formed by multiple small spans. At this time, suppose in one set we have "removeZero" and "(add (padZero l1 l2))", while in the other one we have the "removeZero (add (padZero l1 l2))", NATE still ignore these tokens.\\

\begin{figure}[htbp]
\centerline{\includegraphics[width = \textwidth]{Figures/EX2.2.png}}
\caption{Example code 1.2}
\label{fig:biased case p1}
\end{figure}

Furthermore, it is not surprising that the same issue also arises when its predictions and the ground truth are compared. NATE compensates for this by giving predictions 100\% accuracy if they match completely to any spans in ground truth. This becomes problematic as in Figure \ref{fig:biased case p1}, merely one prediction guesses the empty list highlighted in blue in the ground truth on the left, but NATE gives it 100\% accuracy. Even though this empty list is part of the true source, it is a tiny portion and as a prediction, it is far-off from 100\% accuracy.
